Soft Matching Distance: A metric on neural representations that captures single-neuron tuning

Common measures of neural representational (dis)similarity are designed to be insensitive to rotations and reflections of the neural activation space. Motivated by the premise that the tuning of individual units may be important, there has been recent interest in developing stricter notions of representational (dis)similarity that require neurons to be individually matched across networks. When two networks have the same size (i.e. same number of neurons), a distance metric can be formulated by optimizing over neuron index permutations to maximize tuning curve alignment. However, it is not clear how to generalize this metric to measure distances between networks with different sizes. Here, we leverage a connection to optimal transport theory to derive a natural generalization based on "soft" permutations. The resulting metric is symmetric, satisfies the triangle inequality, and can be interpreted as a Wasserstein distance between two empirical distributions. Further, our proposed metric avoids counter-intuitive outcomes suffered by alternative approaches, and captures complementary geometric insights into neural representations that are entirely missed by rotation-invariant metrics.

==> figures/fig4.tex <==
\begin{SCfigure}
  \centering
  \caption{Soft-matching similarity score effectively captures the alignment of neural tuning. We sample two representations, $\mbX$ and $\mbY$, deliberately varying the extent of alignment in their latent factors (information content) and neural tuning functions, with the color scheme illustrated in A. B and C visualize the changes in alignment between $\mbX$ and $\mbY$ with respect to these manipulated variables, as assessed using $s_\cT$ and CKA, respectively. }
  \includegraphics[width=0.5\textwidth]{figures/fig4.png}%
    \label{fig:4}% picture filename
\end{SCfigure}


% \begin{figure}
% \includegraphics[width=0.7\linewidth]{figures/fig4.png} 
% \centering
% \caption{
%     Simulations verify that the proposed soft-matching similarity score effectively captures the alignment of single-neuron tuning properties. We sample two representations, $\mbX$ and $\mbY$, deliberately varying the extent of alignment in their latent factors (information content) and single-neuron tuning functions (representational form), with the corresponding color scheme illustrated in A. Panels B and C visualize the changes in alignment between $\mbX$ and $\mbY$ with respect to these manipulated variables, as assessed using the soft-matching similarity score ($s_\cT$) and CKA, respectively. }  
% \label{fig:4}
% \end{figure}
